A fast time-domain boundary element method for three-dimensional electromagnetic scattering problems

This paper proposes a fast time-domain boundary element method (TDBEM) to solve three-dimensional transient electromagnetic scattering problems regarding perfectly electric conductors in the classical marching-on-in-time manner. The algorithm of the fast TDBEM is a time-domain variant of the interpolation-based fast multipole method (IFMM), which is similar to the time-domain IFMM for acoustic scattering problems investigated in the author's previous studies. The principle of the present IFMM is to interpolate the kernel functions of the electric and magnetic field integral equations (EFIE and MFIE, respectively) so that every kernel function is expressed in a form of separation of variables in terms of both the spatial and temporal variables. Such an expression enables to construct a fast method to evaluate the scalar and vector potentials in the EFIE and MFIE with using so-called multipole-moments and local-coefficients associated with a space-time hierarchy. As opposed to $O(N_s^2 N_t)$ of the conventional TDBEM, the computational complexity of the fast TDBEM is estimated as $O(N_s^{1+\delta}N_t)$, where $N_s$ and $N_t$ stand for the spatial and temporal degrees of freedom, respectively, and $\delta$ is typically $1/2$ or $1/3$. The numerical examples presented the advantages of the proposed fast TDBEM over the conventional TDBEM when solving large-scale problems.

==> Makefile <==
SRC = ms.tex

TEX = platex
XDVI = pxdvi
DVIPS = pdvips
DVIPDFM = dvipdfmx

BIB = wave3d_paper.bib
AUX = ${SRC:.tex=.aux}
PDF = ${SRC:.tex=.pdf}

yymmdd = $(shell date +%y%m%d_%H%M)

#go: all
#all: ${SRC} ${BIB} 
#	${TEX} ${SRC}
#	makeindex ${SRC:.tex=.nlo} -s nomencl.ist -o ${SRC:.tex=.nls}
#	${TEX} ${SRC}
#	bibtex ${AUX}
all:
	${TEX} ${SRC}
	dvipdfmx ${SRC:.tex=.dvi}
clean:
	rm -f *.dvi *.log *.aux *.lot *.lof *.toc *.blg *.spl *.out core
tar:
	tar cvfz ${SRC:.tex=.tgz} Makefile *.tex *.bib *.sty
euc:
	./sjis2euc.sh *.tex *.sty
sjis:
	./euc2sjis.sh *.tex *.sty
b back backup: tar
	mv ${SRC:.tex=.tgz} backup/${yymmdd}.tgz
	cp -p ${PDF} backup/${yymmdd}.pdf
copy:
	rsync -p 133.6.61.105:/home/ttaka/study/isoel2d/190219/shapeopt/test_circle/*.eps .

response:
	rm -f tmptmptmp*.pdf
	pdfseparate ${PDF} -f 32 -l 35 tmptmptmp%d.pdf
	pdfunite tmptmptmp*.pdf response.pdf
	rm -f tmptmptmp*.pdf
#body:
#	rm -f tmptmptmp*.pdf
#	pdfseparate ${PDF} -f 1 -l 9 tmptmptmp0%d.pdf
#	pdfseparate ${PDF} -f 10 -l 31 tmptmptmp%d.pdf
#	pdfunite tmptmptmp*.pdf ms_revision.pdf
#	rm -f tmptmptmp*.pdf
#source:
#	rm -f source_dir/*
#	cp -p
source:
	tar cvfz source.tar.gz \
	Makefile \
	algorithm.tex   conclusion.tex  fmm.tex         introduction.tex  mydef.tex  tdbem.tex \
	complexity.tex  demo.tex        ms.tex            num.tex    simplify.tex \
	pmbb-sym.sty \
	ms.bbl \
	figure/220905/demo2/bull03_off2off_gimp.eps \
	figure/220905/demo2/bull03-e29953-zoom.eps \
	figure/220905/demo2/X0120_fix_GIMP.eps \
	figure/220905/demo2/X0150_fix_GIMP.eps \
	figure/220905/demo2/X0180_fix_GIMP.eps \
	figure/220905/demo2/X0210_fix_GIMP.eps \
	figure/220905/demo2/X0240_fix_GIMP.eps \
	figure/220905/demo2/X0270_fix_GIMP.eps \
	figure/220905/demo2/X0300_fix_GIMP.eps \
	figure/220905/demo2/X0330_fix_GIMP.eps \
	figure/220905/demo2/X0360_fix_GIMP.eps \
	figure/220905/demo2/bar60_GIMP.eps \
	figure/220905/demo2/fig-bull03-profile-e29953.eps \
	figure/fig-config.eps \
	figure/fig-test-config.eps \
	figure/220905/test8/h03-e4300.eps \
	figure/220905/test8/fig-test-error-dt11add+0-l2.eps \
	figure/220905/test8/fig-h03-e4300-J1.eps \
	figure/220905/test8/fig-h03-e4300-J2.eps \
	figure/220905/test8/fig-h03-e4300-J3.eps \
	figure/220905/test8/fig-test-total-dt11add+0.eps \
	figure/220905/test8/fig-test-memory-dt11add+0.eps \
	figure/220905/test8/fig-test-error-discuss-l2.eps \
	figure/220905/test8/fig-test-error-discuss2-l2.eps \
	figure/fig-problem-modified.eps \
	figure/fig-rwg-basis.eps

#	figure/220905/demo2/X0120_fix.eps \
#	figure/220905/demo2/X0150_fix.eps \
#	figure/220905/demo2/X0180_fix.eps \
#	figure/220905/demo2/X0210_fix.eps \
#	figure/220905/demo2/X0240_fix.eps \
#	figure/220905/demo2/X0270_fix.eps \
#	figure/220905/demo2/X0300_fix.eps \
#	figure/220905/demo2/X0330_fix.eps \
#	figure/220905/demo2/X0360_fix.eps \


h highlight:
	${TEX} highlights.tex
	dvipdfmx highlights.dvi
credit:
	${TEX} credit_author_statement.tex
	dvipdfmx credit_author_statement.dvi

